Deterministic Distributed Expander Decomposition and Routing with Applications in Distributed Derandomization

There is a recent exciting line of work in distributed graph algorithms in the $\mathsf{CONGEST}$ model that exploit expanders. All these algorithms so far are based on two tools: expander decomposition and expander routing. An $(\epsilon,\phi)$-expander decomposition removes $\epsilon$-fraction of the edges so that the remaining connected components have conductance at least $\phi$, i.e., they are $\phi$-expanders, and expander routing allows each vertex $v$ in a $\phi$-expander to very quickly exchange $\text{deg}(v)$ messages with any other vertices, not just its local neighbors. In this paper, we give the first efficient deterministic distributed algorithms for both tools. We show that an $(\epsilon,\phi)$-expander decomposition can be deterministically computed in $\text{poly}(\epsilon^{-1}) n^{o(1)}$ rounds for $\phi = \text{poly}(\epsilon) n^{-o(1)}$, and that expander routing can be performed deterministically in $\text{poly}(\phi^{-1})n^{o(1)}$ rounds. Both results match previous bounds of randomized algorithms by [Chang and Saranurak, PODC 2019] and [Ghaffari, Kuhn, and Su, PODC 2017] up to subpolynomial factors. Consequently, we derandomize existing distributed algorithms that exploit expanders. We show that a minimum spanning tree on $n^{o(1)}$-expanders can be constructed deterministically in $n^{o(1)}$ rounds, and triangle detection and enumeration on general graphs can be solved deterministically in $O(n^{0.58})$ and $n^{2/3 + o(1)}$ rounds, respectively. We also give the first polylogarithmic-round randomized algorithm for constructing an $(\epsilon,\phi)$-expander decomposition in $\text{poly}(\epsilon^{-1}, \log n)$ rounds for $\phi = 1 / \text{poly}(\epsilon^{-1}, \log n)$. The previous algorithm by [Chang and Saranurak, PODC 2019] needs $n^{\Omega(1)}$ rounds for any $\phi\ge 1/\text{poly}\log n$.

==> loadbalancing.tex <==

\section{Deterministic Load Balancing in Expanders}\label{sect-load-bal}
\thatchaphol{Mention related techniques here in and also in the technical overview. Does the potential appear before? If so, in which context? Say that will be used for routing. Can be of independent interest (hence a separated section). 
IMPORTANT: Can use Theorem 3.5 of \cite{GhoshLMMPRRTZ99} as a blackbox.}
Consider a graph $G=(V,E)$ with $\Phiv(G) \geq \psi$, and $n$ is the number of vertices, and $\Delta$ is the maximum degree. Suppose each vertex $v \in V$ initially has $t_v$ tokens. Let $L = \sum_{v \in V} t_v / n$ be the average load, and let $M =\max_{v \in V} t_v$ be the maximum load. We show that there is an $O(\psi^{-1} \Delta^{-1} M^2)$-round algorithm that redistributes the tokens in such a way that the maximum load at a vertex is at most $2L + O(\psi^{-1} \Delta^2  \log n)$.

\begin{lemma}[{Load balancing~\cite[Theorem 3.5]{GhoshLMMPRRTZ99}}]\label{lem-loadbal-main}
There is an $O(\psi^{-1} M)$-round deterministic algorithm that redistribute the tokens in such a way that the maximum load at a vertex is  at most $L + O(\psi^{-1} \Delta^2  \log n)$. During the algorithm, at most one token is sent along each edge in each round.
%There is an $O(\psi^{-1} \Delta^{-1} M^2)$-round deterministic algorithm that redistribute the tokens in such a way that the maximum load at a vertex is  at most $2L + O(\psi^{-1} \Delta^2  \log n)$. During the algorithm, at most one token is sent along each edge in each round.
\end{lemma}


Given the current token distribution $\mu = (t_1, t_2, \ldots, t_n)$, where $t_i$ is the number of tokens at $v_i$, we define the potential function $\Pi(\mu) = \sum_{1 \leq i \leq n} \Pi(t_i)$, where $\Pi(x) = {(1 + (\psi \Delta^{-2} / 10))}^{x}$. 
Let $M_{\mu} = \max_{1 \leq i \leq n} t_i$. We assume $M_{\mu} = 2L + \Omega(\psi^{-1}\Delta^{ 2} \log n)$, since otherwise we are done already. We write $S_j$ to denote the set of indices such that $t_i \geq j$.

Consider the following algorithm that updates $\mu$ to $\mu'$.
\begin{enumerate}
    \item For each $0 \leq j \leq M$, define $a_j = |S_j| \cdot  \Pi(j)$. Select $j^\ast$ to be $\arg \max_{1 \leq j \leq M} a_j$.
    \item We say that an edge $e = \{v_i, v_k\}$ is \emph{good} if  $i \in S_{j^\ast}$ and $t_k \leq t_i - (3\Delta+1)$. For each good edge  $e = \{v_i, v_k\}$, send 1 token from $v_i$ to $v_k$, in parallel.
\end{enumerate}
Note that in the above algorithm, some vertices might increase or decrease its number of tokens by at most $\Delta$. The goal of the analysis is to show that as long as  $M_{\mu} \geq 2L + \Omega(\psi^{-1}\Delta^{2} \log n)$, the potential decrease is $\Pi(\mu) - \Pi(\mu') =  \Omega(\psi^2 \Delta^{-1} M^{-1}) \cdot \Pi(\mu)$, and then we can use this to upper bound the number of iterations.

\begin{lemma}\label{lem-loadbal-1}
We have $j^\ast =  M_{\mu} - O(\psi^{-1}\Delta^{2} \log n)  > 2L$, and so $|S_{j^\ast}| < n/2$.
\end{lemma}
\begin{proof}
We can upper bound any $a_j$ by $n \cdot \Pi(j)$.
Since $\Pi(j) = \Pi(M_{\mu}) \cdot {(1 + (\psi \Delta^{-2} / 10))}^{M_{\mu} - j}$, if $M_{\mu} - j \geq 1.1 (\ln n) / (\psi \Delta^{-2} / 10)$, then $\Pi(j) < (1/n) \Pi(M_{\mu})$, which implies that $a_j <  a_{M_{\mu}}$. Therefore, we need to have $j^\ast = M_{\mu} - O(\psi^{-1}\Delta^{2} \log n)  > 2L$, and it immediately implies that 
 $|S_{j^\ast}| <  n/2$, as $L$ is the average load.
\end{proof}


\begin{lemma}\label{lem-loadbal-2}
The number of tokens being sent in an iteration is $\Omega(\psi) \cdot |S_{j^\ast}|$.
\end{lemma}
\begin{proof}
Define $W = S_{j^\ast - 3\Delta} \setminus S_{j^\ast}$. We claim that $|W| \leq (\psi \Delta^{-1}/2) |S_{j^\ast}|$. Suppose  $|W| > (\psi \Delta^{-1} /2) |S_{j^\ast}|$. Then we have
\begin{align*}
a_{j^\ast - 3\Delta} 
&> (1 + (\psi \Delta^{-1}/2)) |S_{j^\ast}| \Pi(j^\ast - 3\Delta)\\
&= (1 + (\psi \Delta^{-1}/2)) |S_{j^\ast}| {(1 + (\psi \Delta^{-2} / 10))}^{j^\ast - 3\Delta}\\
&= (1 + (\psi \Delta^{-1}/2)) {(1 + (\psi \Delta^{-2} / 10))}^{- 3\Delta} a_{j^\ast}\\
&> (1 + (\psi \Delta^{-1}/2)) (1 + (\psi \Delta^{-1}/3))^{-1} a_{j^\ast}\\
&> a_{j^\ast},
\end{align*}
which is a contradiction to the choice of $j^\ast$.
Note that an edge $e = \{v_i, v_k\}$ is good if $v_i \in S_j$ and $v_k \notin W$. We show that the number of good edges is $\Omega(\psi \Delta^{-1}) \cdot |S_{j^\ast}|$.
Since $G$ has sparsity $\Phiv(G) \geq \psi$ and $|S_{j^\ast}| < n/2$ (\cref{lem-loadbal-1}), we have $|\partial(S_{j^\ast})| \geq \psi |S_{j^\ast}|$. Among the edges in $\partial(S_{j^\ast})$, at least $\psi |S_{j^\ast}| - |W|\Delta \geq  (\psi/2) |S_{j^\ast}|$ of these edges are good.
\end{proof}

To analyze the potential decrease, instead of sending the tokens in parallel, we process them sequentially in the analysis. 


\begin{lemma}\label{lem-loadbal-3}
If $t_k \leq t_i - (\Delta+1)$, then
sending 1 token from $v_i$ to $v_k$ results in an overall potential decrease of $\Omega(\psi \Delta^{-1}) \cdot \Pi(t_i)$
\end{lemma}
\begin{proof}
We write $x = t_i - t_l \geq \Delta+1$.
Initially, the summation of the potential of $v_i$ and $v_k$ is \[\Pi(t_i) + \Pi(t_k) = 1 + {(1 + (\psi \Delta^{-2} / 10))}^{-x} \cdot \Pi(t_i).\]
After the token transfer, the  summation of the potential of $v_i$ and $v_k$ becomes \[\left( {(1 + (\psi \Delta^{-2} / 10))}^{-1} + {(1 + (\psi \Delta^{-2} / 10))}^{-(x-1)}\right) \cdot \Pi(t_i).\] We need to show that
\[
{1 + {(1 + (\psi \Delta^{-2} / 10))}^{-x} - (1 + (\psi \Delta^{-2} / 10))}^{-1} - {(1 + (\psi \Delta^{-2} / 10))}^{-(x-1)} = \Omega(\psi \Delta^{-1}).
\]
Considering its Taylor series, we see that it is at least $(x-2) (\psi \Delta^{-2} / 10)) (1 - o(1)) = \Omega(\psi \Delta^{-1})$.\end{proof}

\begin{lemma}\label{lem-loadbal-4}
The overall potential decrease in one iteration is $\Omega(\psi^2 \Delta^{-1} M^{-1}) \cdot \Pi(\mu)$.
\end{lemma}
\begin{proof}
In view of \cref{lem-loadbal-2,lem-loadbal-3}, the overall  potential decrease in one iteration is $\Omega(\psi \Delta^{-1}) \cdot \Omega(\psi) \cdot |S_{j^\ast}| \cdot \Pi(t_{j^\ast}) = \Omega(\psi^2 \Delta^{-1}) \cdot a_{j^\ast}$. To prove this lemma, it suffices to show that $a_{j^\ast} = \Omega(1/M) \cdot \Pi(\mu)$. This follows from the observation that $\Pi(\mu) \leq a_0 + a_1 + \cdots + a_M$ and our choice of $j^\ast$.
\end{proof}



\begin{lemma}\label{lem-loadbal-5}
The number of iterations needed to reduce the maximum load per vertex to $2L + O(\psi^{-1}\Delta^2  \log n)$ is $O(\psi^{-1} \Delta^{-1} M^2)$.
\end{lemma}
\begin{proof}
We can upper bound the initial potential by $A = n \cdot \Pi(M) = n \cdot \Pi(M)$.
By \cref{lem-loadbal-4}, we can upper bound the number of iterations by $x = \log_{1+B} A$, where $B = \Omega(\psi^2 \Delta^{-1} M^{-1})$. A simple calculation shows that $x = O(\psi^{-2} \Delta M) \cdot O( M \psi \Delta^{-2} + \log n) = O(\psi^{-1} \Delta^{-1} M^2)$.
Note that we use the fact $M = \Omega(\psi^{-1}\Delta^2 \log n)$ in the above calculation.
\end{proof}

Now we consider the distributed implementation. 
Observe that we can use the following simpler algorithm. In each iteration  simultaneously for each edge $e = \{v_i, v_j\}$, check if $t_i \geq t_j - (3 \Delta + 1)$, and send a token from $v_i$ to $v_j$ if this inequality holds. It is straightforward to see that the overall potential decrease of one iteration of this algorithm is at least as good as the previous one. Thus, we conclude  \cref{lem-loadbal-main}.  
\thatchaphol{I want to conjecture that this algorithm terminate in $O(\psi^{-1}\Delta^{-1}M)$ rounds instead of $O(\psi^{-1}\Delta^{-1}M^2)$. Currently, this reason there is an additional factor of $M$ is because we are only focusing on $j^*$. }


